Efficient $\ell^0$ gradient-based Super Resolution for simplified image segmentation

We consider a variational model for single-image super-resolution based on the assumption that the gradient of the target image is sparse. We enforce this assumption by considering both an isotropic and an anisotropic $\ell^0$ regularisation on the image gradient combined with a quadratic data fidelity, similarly as studied in [1] for general signal recovery problems. For the numerical realisation of the model, we propose a novel efficient ADMM splitting algorithm whose substeps solutions are computed efficiently by means of hard-thresholding and standard conjugate-gradient solvers. We test our model on highly-degraded synthetic and real-world data and quantitatively compare our results with several variational approaches as well as with state-of-the-art deep-learning techniques. Our experiments show that $\ell^0$ gradient-regularised super-resolved images can be effectively used to improve the accuracy of standard segmentation algorithms when applied to QR and cell detection, and landcover classification problems, in comparison to the results achieved by other approaches.

==> section/theorem_old.tex <==
\section{Convergence analysis} \label{sec:convergence}

We report here the convergence proofs of Theorem \ref{th:conv_ADMManiso} and Theorem \ref{th:conv_ADMMiso}. We provide a detailed proof for Theorem \ref{th:conv_ADMManiso} while providing only few details for Theorem \ref{th:conv_ADMMiso} whose proof is based on essentially the same arguments.

\subsection{Proof of Theorem \ref{th:conv_ADMManiso}}
We consider the ADMM sequences $(\ubold^{k}),(\tbold^{k}),(\sbold^{k})$, defined in \eqref{eq:ADMM_aniso_1}-\eqref{eq:ADMM_aniso_3}. We want to show that there exists $\ubold^*$ such that:
\begin{align}
\ubold^{k} \rightarrow \ubold^{*}, \quad \tbold^{k} \rightarrow\Dbold_{h}\ubold^{*}\nonumber, \quad \sbold^{k} \rightarrow  \Dbold_{v}\ubold^{*}. 
\end{align}
\textcolor{red}{To shorten the proof, we remark that everything proved for the sequences $(\tbold^{k})$,$(\beta_{t}^{k})$, $(\boldsymbol{\lambda}_{t}^{k})$ and $(\Dbold_{h}\ubold^{k})$ can be deduced for $(\sbold^{k})$, $(\beta_{s}^{k})$, $(\boldsymbol{\lambda}_{s}^{k})$ and $(\Dbold_{v}\ubold^{k})$, respectively.}

We start defining the following functionals:
\begin{align*}
&G^{h}_{k}(\tbold):= \mu \lVert \tbold \rVert_{0} + \dfrac{\beta_{t}^{k}}{2} \lVert \tbold - (\Dbold_{h}\ubold^{k}+\dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}})\rVert_{2}^{2}, \\
%&G^{v}_{k}(\sbold):= \mu \lVert \sbold \rVert_{0} + \dfrac{\beta_{s}^{k}}{2} \lVert \sbold - (\Dbold_{v}\ubold^{k}+\dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}})\rVert_{2}^{2},  \\
& F_{k}(\ubold):= \dfrac{1}{2}\lVert \Sbold \Hbold \ubold - \gbold \rVert_{2}^{2}  + \dfrac{\beta_{t}^{k}}{2}\lVert \Dbold_{h}\ubold - (\tbold^{k+1} - \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}})\rVert^{2}_{2} + \nonumber \\  & + \dfrac{\beta_{s}^{k}}{2}\lVert \Dbold_{v}\ubold - (\sbold^{k+1} - \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}})\rVert^{2}_{2}.
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph*{Step 1}
There holds: 
\begin{align}
&\lVert \tbold^{k+1} -\Dbold_{h}\ubold^{k} - \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \rVert_{2} \leq \sqrt{\dfrac{2 \mu N}{\beta_{t}^{k}}}. \label{proof:step1_limitato_t} %\\
%&\lVert \sbold^{k+1} -\Dbold_{v}\ubold^{k} - \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}} \rVert_{2}^{2} \leq \dfrac{2 \mu N}{\beta_{s}^{k}}. \label{proof:step1_limitato_s}
\end{align}
\textcolor{red}{This inequality} can  be trivially shown by the minimality of $\tbold^{k+1}$ in \eqref{eq:ADMM_aniso_1} which entails   $G^{h}_{k}(\tbold^{k+1}) \leq  G^{h}_{k}(\Dbold_{h}\ubold^{k} + \frac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}})$, therefore we get:
\begin{align*}
& \mu \lVert \tbold^{k+1}\rVert_{0} + \dfrac{\beta_{t}^{k}}{2} \lVert \tbold^{k+1} - (\Dbold_{h}\ubold^{k}+\dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}})\rVert_{2}^{2} \notag\\
& \leq \mu \lVert \Dbold_{h}\ubold^{k} + \frac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \rVert_{0} \leq \textcolor{red}{\mu} N,
\end{align*}
by definition of $\lVert \cdot \rVert_0$. We remark that $N$ is the size of $ubold^{k}$. By neglecting the first term on the Left Hand Side (LHS)  of the above inequality \textcolor{red}{and applying the square root} we deduce \eqref{proof:step1_limitato_t}. %From \eqref{proof:step1_limitato_t} and since $(\beta_t^k)\nearrow +\infty$ we have:
%\begin{align}
%&\lVert \tbold^{k+1} -\Dbold_{h}\ubold^{k} - \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \rVert_{2}^{2} \rightarrow 0  \label{proof:step1_infinitesimo_t},\\
%&\lVert \sbold^{k+1} -\Dbold_{v}\ubold^{k} - \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}} \rVert_{2}^{2} \rightarrow 0 \label{proof:step1_infinitesimo_s}
%\end{align}
%\begin{align}
%&\lVert \tbold^{k+1} -\Dbold_{h}\ubold^{k} - \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \rVert_{2}^{2} \rightarrow 0 \label{proof:step1_infinitesimo_s} %, \lVert \sbold^{k+1} -\Dbold_{v}\ubold^{k} - \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}} \rVert_{2}^{2} \rightarrow 0 
%\end{align}

\paragraph*{Step 2}
From the minimality of $\ubold^{k+1}$ in \eqref{eq:ADMM_aniso_3} we have: $F_{k}(\ubold^{k+1}) \leq F_{k}(\ubold^{k})$ for every $k$. By definition of $F_{k}$ and applying \eqref{proof:step1_limitato_t} and \textcolor{red}{its counterpart related to the sequences $(\sbold^{k})$, $(\beta_{s}^{k})$, $(\boldsymbol{\lambda}_{s}^{k})$ and $(\Dbold_{v}\ubold^{k})$}, we deduce: 
\begin{align}
    & \dfrac{1}{2}\lVert \Sbold \Hbold \ubold^{k+1} - \gbold \rVert_{2}^{2}  + \dfrac{\beta_{t}^{k}}{2} \lVert \Dbold_{h} \ubold^{k+1} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \rVert_{2}^{2} + \nonumber \\
    & + \dfrac{\beta_{s}^{k}}{2} \lVert \Dbold_{v} \ubold^{k+1} - \sbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}}  \rVert_{2}^{2} \leq  \label{proof:riferimento} \\
    & \dfrac{1}{2}\lVert \Sbold \Hbold \ubold^{k} - \gbold \rVert_{2}^{2}  + \dfrac{\beta_{t}^{k}}{2} \lVert \Dbold_{h} \ubold^{k} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \rVert_{2}^{2} + \nonumber \\
    & + \dfrac{\beta_{s}^{k}}{2} \lVert \Dbold_{v} \ubold^{k} - \sbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}}  \rVert_{2}^{2} \leq \dfrac{1}{2}\lVert \Sbold \Hbold \ubold^{k} - \gbold \rVert_{2}^{2} + 2\mu N \nonumber.
\end{align}


Since the all the terms in the LHS of \eqref{proof:riferimento} are nonnegative, also the following inequality holds: 
\begin{align}
    & \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{k+1} -\gbold \rVert_{2}^{2} \leq \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{k} -\gbold \rVert_{2}^{2} + 2 \mu N,  \nonumber
\end{align}
which can be recursively iterated, thus getting the following relation  for every $k\geq 1$:
\begin{align*}
  \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{k} -\gbold \rVert_{2}^{2} \leq \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{0} - \gbold \rVert_{2}^{2} +  2 \mu N k.
\end{align*} 

%In the following, we focus on the convergence of the sequence ($\tbold^{k}$), then we can similarly proceed for the sequence ($\sbold^{k}$).  

From \eqref{proof:riferimento} we can also derive the following inequality (due again to the nonnegativity of all the three terms in the  LHS):
\begin{align}
    & \dfrac{\beta_{t}^{k}}{2} \lVert \Dbold_{h} \ubold^{k+1} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \rVert_{2}^{2} \leq \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{k} -\gbold \rVert_{2}^{2} + 2 \mu N,  \nonumber
\end{align}
and using the estimate above, we can deduce the following:

\begin{align*}
    & \dfrac{\beta_{t}^{k}}{2} \lVert \Dbold_{h}\ubold^{k+1} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}}\rVert^{2}_{2}  \leq \nonumber \\
    &  \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{k} - \gbold \rVert_{2}^{2} + 2 \mu N \leq \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{0} - \gbold \rVert_{2}^{2} +  2 \mu N k , 
%    &  \dfrac{\beta_{s}^{k}}{2} \lVert \Dbold_{v}\ubold^{k+1} - \sbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}}\rVert^{2}_{2}  \leq \nonumber \\
%    &  \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{k} - \gbold  \rVert_{2}^{2} + 2 \mu N \leq \dfrac{1}{2} \lVert \Sbold \Hbold \ubold^{0} - \gbold \rVert_{2}^{2} + 2 \mu N k \label{proof:36}
\end{align*}
which entails:
\begin{align}\label{ineq:series_convergent2}
\textcolor{red}{\lVert \Dbold_{h}\ubold^{k+1} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}}\rVert_{2}  \leq \sqrt{\frac{1}{{\beta_{t}^{k}}}}\lVert \Sbold \Hbold \ubold^{0} - \gbold \rVert_{2} + \sqrt{4\mu N \frac{k}{\beta_{t}^{k}}}}. 
\end{align}

By assumption \ref{cond:1_ADMManiso} we get  $(\beta_t^k)\nearrow +\infty$ and $\dfrac{k}{\beta^{k}_{t}} \rightarrow 0$, then it follows:
\begin{align} 
    &\lVert \Dbold_{h}\ubold^{k+1} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}}\rVert_{2} \rightarrow 0. \label{prof:bound1}%\\
    %&\lVert \Dbold_{v}\ubold^{k+1} - \sbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}}\rVert^{2}_{2} \rightarrow 0 \label{prof:bound2}
\end{align}
%and, similarly, that:
%\begin{align*} 
    %&\lVert \Dbold_{h}\ubold^{k+1} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}}\rVert^{2}_{2} \rightarrow 0 \label{prof:bound1}%\\
%    &\lVert \Dbold_{v}\ubold^{k+1} - \sbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}}\rVert^{2}_{2} \rightarrow 0. 
%\end{align*}

\paragraph*{Step 3}
We show that the sequences $\Dbold_{h}\ubold^{k}$ ans $\Dbold_{v}\ubold^{k}$ are Cauchy sequences, hence they converge. We prove this for $\Dbold_{h}\ubold^{k}$, the proof for $\Dbold_{v}\ubold^{k}$ is identical.
\begin{align*}
    & \lVert \Dbold_{h} \ubold^{k+1} - \Dbold_{h} \ubold^{k} \rVert_{2} \leq \nonumber \\
    &\leq \lVert \Dbold_{h}\ubold^{k+1} - \tbold^{k+1} +  \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}}  \rVert_{2}  +   \lVert \Dbold_{h}\ubold^{k} - \tbold^{k+1} +  \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}}  \rVert_{2} . 
\end{align*}
By assumption \ref{cond:1_ADMManiso} we get $\sum_{k=0}^{+\infty} \sqrt{\frac{1}{\beta^{k}_{t}}} < + \infty$. Therefore, from \eqref{proof:step1_limitato_t} and \eqref{ineq:series_convergent2} $\Dbold_{h}\ubold^{k}$ is a Cauchy sequence, which thus converges to a point $\tbold^{*}$. Similarly, $\Dbold_{v}\sbold^{k}$ which converges to some $\sbold^{*}$.

%and by assumption \eqref{cond:1_ADMManiso} the RHS tends to  $0$ as $k\to +\infty$, As a consequence,

\paragraph*{Step 4}
We start rewriting \eqref{eq:ADMM_aniso_4}: 
\begin{align}
 &\frac{\boldsymbol{\lambda}_{t}^{k+1}}{\beta_{t}^{k}} = \Dbold_{h} \ubold^{k+1} - \tbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}}. \label{eq:proof_dual1}%\\
%&\frac{\boldsymbol{\lambda}_{s}^{k+1}}{\beta_{s}^{k}} = \Dbold_{v} \ubold^{k+1} - \sbold^{k+1} + \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}}.  \label{eq:proof_dual2}
\end{align}
By \eqref{prof:bound1}, the RHS of this equation tends to $0$ as $k\to \infty$, whence we deduce that $\frac{\lVert \boldsymbol{\lambda}_{t}^{k+1} \rVert_{2}}{\sqrt{\beta_{t}^{k}}} \rightarrow 0 $. By monotonicity of the $(\beta^k_t)$ we then deduce that  $\frac{\lVert \boldsymbol{\lambda}_{t}^{k} \rVert_{2}}{\sqrt{\beta_{t}^{k}}} \rightarrow 0 $. Hence:
\begin{align*}
& \lVert \Dbold_{h}\ubold^{k+1} - \tbold^{k+1} \rVert_{2} \leq  \dfrac{\lVert \boldsymbol{\lambda}_{t}^{k+1}\rVert_{2} + \lVert \boldsymbol{\lambda}_{t}^{k}\rVert_{2}}  {\sqrt{\beta_{t}^{k}}}, 
% \\
% & \lVert \Dbold_{v}\ubold^{k+1} - \sbold^{k+1} \rVert_{2} \leq  \dfrac{\lVert \boldsymbol{\lambda}_{s}^{k+1}\rVert_{2} + \lVert \boldsymbol{\lambda}_{s}^{k}\rVert_{2}}  {\sqrt{\beta_{s}^{k}}}, 
\end{align*}
where both quantities on the RHS tend to $0$ as $k\to\infty$. Therefore, $\tbold^{k}$ converges to $\tbold^{*}$ as well as $\Dbold_{h}\ubold^{k}$  and $\sbold^{k}$ converges to $\sbold^{*}$ as well as $\Dbold_{v}\ubold^{k}$, by uniqueness of the limit.

\paragraph*{Step 5}
We can now prove the convergence of $\ubold^{k}$ . For simplicity, let us define the quantities $\Abold:=\Sbold\Hbold$ and  $\Mbold_{k}:=\dfrac{1}{\beta_t^{k}} \Abold^{T}\Abold + \Dbold_{h}^{T}\Dbold_{h} + \dfrac{\beta_{s}^{k}}{\beta_{t}^{k}}\Dbold_{v}^{T}\Dbold_{v}$, for every $k$. \textcolor{red}{Since \ref{cond:2_ADMManiso} holds}, we observe that the matrix $\Mbold_k$ is invertible and symmetric for all $k$. The optimality condition of problem \eqref{eq:ADMM_aniso_3} reads:
\begin{equation}
\Mbold_{k}\ubold^{k}= \Dbold_{h}^{T} (\tbold^{k+1} - \dfrac{\boldsymbol{\lambda}_{t}^{k}}{\beta^{k}}) + \dfrac{\beta_{s}^{k}}{\beta_{t}^{k}}\Dbold_{v}^{T}(\sbold^{k+1} - \dfrac{\boldsymbol{\lambda}_{s}^{k}}{\beta^{k}}) + \dfrac{1}{\beta_{t}^{k}}\Abold^{T}\gbold. \nonumber
\end{equation}

Since $\tbold^{k+1} \to \tbold^{*}$, $\sbold^{k+1} \to \sbold^{*}$,  $\frac{\boldsymbol{\lambda}_{t}^{k}}{\beta_{t}^{k}} \to 0$, $\frac{\boldsymbol{\lambda}_{s}^{k}}{\beta_{s}^{k}} \to 0$ by the previous steps, $\Dbold_{h}^{T}$ and $\Dbold_{v}^{T}$ are continuous operators, $\frac{\beta_{s}^{k}}{\beta_{t}^{k}} \to c$ by hypothesis, and  $\frac{1}{\beta_{t}^{k}}\Abold^{T}\gbold \to 0$ by the assumption $(\beta_t^k)\nearrow +\infty$, then the RHS converges pointwise to $\zbold^{*}=\Dbold_{h}^{T}t^{*} + c \Dbold_{v}^{T}s^{*} $. Therefore, $\Mbold_{k}u^{k} \to \zbold^{*}$. Additionally, the sequence $\Mbold_{k}^{-1}$ converges pointwise to a continuous operator $\Mbold^{*}$. We thus have that $\Mbold_{k}^{-1}\Mbold_{k}\ubold^{k} \to \Mbold^{*}\zbold^{*}$, or equivalently, $\ubold^{k} \to \Mbold^{*}\zbold^{*}:=\ubold^{*}$. We now want to show that $\tbold^*=\Dbold_h \ubold^*$ and, similarly, that $\sbold^*=\Dbold_v \ubold^*$. We show the details only for the former case. By the triangle inequality we get:
\begin{align}
\lVert \tbold^* -  \Dbold_h \ubold^*\rVert_2  \leq & \lVert \tbold^* -  \Dbold_h \ubold^k\rVert_2 + \lVert \Dbold_h \ubold^k - \Dbold_h \ubold^* \rVert_2 \nonumber \\
& \lVert \tbold^* -  \Dbold_h \ubold^k\rVert_2 + \lVert \Dbold_h \rVert \lVert \ubold^k - \ubold^* \rVert_2, \nonumber
\end{align}
where the both terms tend to $0$ by what shown in Step 3 and above. This concludes the proof.

%The sequence $\Mbold_{k}\ubold^{k}$ converges since the right and side converges. Since we are in finite dimension and $\Dbold_{h}$, $\Dbold_{v}$ are full-rank we can say that $\ubold^{k}$ converges to $\ubold^{*}$. 


%Since $\Dbold_{h}\ubold^{k}$ and $\Dbold_{v}\ubold^{k}$ converge to $\tbold^{*}$ and $\sbold^{*}$, respectively, and  $\Dbold_{h}\ubold^{k}$ and $\Dbold_{v}\ubold^{k}$ converge to $\Dbold_{h}\ubold^{*}$ and $\Dbold_{v}\ubold^{*}$, respectively, it follows that are $\tbold^{*}=\Dbold_{h}\ubold^{*}$ $\sbold^{*}\Dbold_{v}\ubold^{*}$.

\subsection{Proof of Theorem \eqref{th:conv_ADMMiso}}

The proof of Theorem \eqref{th:conv_ADMMiso} follows the same steps as the previous one. The only main difference in it is the definiton of $\Mbold_{k}$, which reads in this case:
\begin{align}
    \Mbold_{k}:= \dfrac{1}{\beta^{k}} \Abold^{T}\Abold + \Dbold^{T}\Dbold =
    \dfrac{1}{\beta^{k}} \Abold^{T}\Abold+
    \Dbold_{h}^{T}\Dbold_{h} + \Dbold_{v}^{T}\Dbold_{v}. \nonumber
\end{align}
By proceeding similarly as above the conclusion holds.
